Hadronic Footprint of GeV-Mass Dark Matter

GeV-scale dark matter is an increasingly attractive target for direct detection, indirect detection, and collider searches. Its annihilation into hadronic final states produces a challenging zoo of light hadronic resonances. We update Herwig7 to study the photon and positron spectra from annihilation through a vector mediator. It covers dark matter masses between 250 MeV and 5 GeV and includes an error estimate.

==> paper/incl_declare.tex <==

%\definecolor{Gcolor}{HTML}{3b528b}
%\definecolor{Dcolor}{HTML}{e41a1c}

%\tikzstyle{generator} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=Gcolor]
%\tikzstyle{discriminator} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=Dcolor]
%\tikzstyle{io} = [circle, trapezium left angle=70, trapezium right angle=110, minimum width=1cm, minimum height=1cm, text centered, draw=black]

%\tikzstyle{process} = [rectangle, minimum width=1cm, minimum height=1cm, text centered, draw=black]
%\tikzstyle{decision} = [rectangle, minimum width=1cm, minimum height=1cm, text centered, draw=black]

%\tikzstyle{arrow} = [thick,->,>=stealth]
%\usepackage{xcolor}

%% macros for marking changes
%\marginparwidth 3.0cm
%\setlength{\hoffset}{-1.6cm}
%\newcommand{\mpar}[1]{\rule{2pt}{10pt}
%                      {\marginpar{\hbadness10000\flushleft
%                      \sloppy\hfuzz10pt\boldmath\footnotesize#1}}
%                       \typeout{marginpar: #1}\ignorespaces}
%\def\mda{\mpar{\hfil$\downarrow$\hfil}\ignorespaces}
%\def\mua{\mpar{\hfil$\uparrow$\hfil}\ignorespaces}
%\def\mla{\marginpar[\boldmath\hfil$\rightarrow$\hfil]
%                   {\boldmath\hfil$\leftarrow $\hfil}
%                    \typeout{marginpar: $\leftrightarrow$}\ignorespaces}

% hyper-link hep-ph references
%\newcommand{\arxiv}[1]{\href{http://arxiv.org/abs/#1}{arXiv:#1}}
%\newcommand{\urlx}[1]{\href{#1}{#1}}
%\newcommand{\doix}[2]{\href{http://dx.doi.org/#2}{#1}}

\setlength{\tabcolsep}{2pt}

%\newcommand*{\thead}[1]{\multicolumn{1}{c}{\bfseries #1}}

\def\contentsname{{\normalsize Content}}
\def\tablename{Table}
\def\figurename{Figure}

\newcommand{\Langle}{\big\langle}
\newcommand{\Rangle}{\big\rangle}

\newcommand{\psib}{\overline{\psi}}
\newcommand{\Psib}{\overline{\Psi}}
%\newcommand{\dslash}{\not{\hbox{\kern-3pt $\partial$}}}
%\newcommand{\Dslash}{\not{\hbox{\kern-3pt $D$}}}
%\def\one{\leavevmode\hbox{\small1\kern-7.3pt\normalsize1}}
%%\def\one{I}
\newcommand\one{\leavevmode\hbox{\small1\normalsize\kern-.33em1}}
\newcommand{\Mpl}{M_\text{Pl}}
\newcommand{\mdm}{m_\chi}
%\def\dslash{\not{\hbox{\kern-4pt $\partial$}}}
%\def\Dslash{\not{\hbox{\kern-4pt $D$}}}
\newcommand{\p}{\partial}
\newcommand{\mat}{\mathcal{M}}
\newcommand{\lag}{\mathcal{L}}
\newcommand{\ord}{\mathcal{O}}
\newcommand{\ope}{\mathcal{O}}
\newcommand{\matx}{|\mathcal{M}|^2}

\newcommand{\qqquad}{\qquad \qquad}
\newcommand{\qqqquad}{\qquad \qquad \qquad}

\newcommand{\qb}{\bar{q}}
\newcommand{\really}{\stackrel{!}{=}}
\newcommand{\msbar}{\overline{\text{MS}}}
\newcommand{\qns}{f_q^\text{NS}}
\newcommand{\lqcd}{\Lambda_\text{QCD}}
\newcommand{\met}{\slashchar{E}_T}
\newcommand{\pmiss}{\slashchar{\vec{p}}_T}

% for SUSY fit projects
\newcommand{\Mzero}{\ensuremath{m_0}}
\newcommand{\MOneHalf}{\ensuremath{m_{1/2}}}
\newcommand{\omegacdm}{\ensuremath{\Omega h^2}}
\newcommand{\Mtop}{\ensuremath{m_t}}
\newcommand{\Mone}{\ensuremath{M_1}}
\newcommand{\Mtwo}{\ensuremath{M_2}}
\newcommand{\Mthree}{\ensuremath{M_3}}
\newcommand{\Deltaamu}{\ensuremath{\text{\Delta a_\mu}}}
\newcommand{\chisq}{{\ensuremath -2\log L}}
\newcommand{\Alambda}{{\ensuremath {A_\lambda}}}
\newcommand{\Akappa}{{\ensuremath {A_\kappa}}}
\newcommand{\tkappa}{{\ensuremath{\tilde \kappa}}}
\newcommand{\abs}[1]{\left |#1\right |}
\newcommand{\unit}[1]{\ensuremath{\, \text{#1}}}

\newcommand{\lsp}{\tilde \chi}
\newcommand{\sq}{\tilde{q}}
\newcommand{\go}{\tilde{g}}
\newcommand{\st}[1]{\tilde{t}_{#1}}
\newcommand{\stb}[1]{\tilde{t}_{#1}^*}
\newcommand{\nz}[1]{\tilde{\chi}_{#1}^0}
\newcommand{\cp}[1]{\tilde{\chi}_{#1}^+}
\newcommand{\cm}[1]{\tilde{\chi}_{#1}^-}
\newcommand{\CP}{CP}

% all the masses 
\providecommand{\mg}{m_{\tilde{g}}}
\providecommand{\mst}[1]{m_{\tilde{t}_{#1}}}
\newcommand{\msn}[1]{m_{\tilde{\nu}_{#1}}}
\newcommand{\mch}[1]{m_{\tilde{\chi}^+_{#1}}}
\newcommand{\mne}[1]{m_{\tilde{\chi}^0_{#1}}}
\newcommand{\msb}[1]{m_{\tilde{b}_{#1}}}
\newcommand{\vsm}{\ensuremath{v_\text{SM}}}

% units of measure
\newcommand{\cmu}{\text{cm}}
\newcommand{\mev}{\text{MeV}}
\newcommand{\gev}{\text{GeV}}
\newcommand{\tev}{\text{TeV}}
\newcommand{\fb}{\text{fb}}
\newcommand{\ab}{\text{ab}}
\newcommand{\pb}{\text{pb}}
\newcommand{\br}{\text{BR}}
\newcommand{\sign}{\text{sign}}
\newcommand{\ifb}{\ensuremath{\text{fb}^{-1}} }
\newcommand{\iab}{\ensuremath{\text{ab}^{-1}} }
\newcommand{\ipb}{\text{pb}^{-1}}

% really great macro by Chris Lester
\def\slashchar#1{\setbox0=\hbox{$#1$}           % set a box for #1
   \dimen0=\wd0                                 % and get its size
   \setbox1=\hbox{/} \dimen1=\wd1               % get size of /
   \ifdim\dimen0>\dimen1                        % #1 is bigger
      \rlap{\hbox to \dimen0{\hfil/\hfil}}      % so center / in box
      #1                                        % and print #1
   \else                                        % / is bigger
      \rlap{\hbox to \dimen1{\hfil$#1$\hfil}}   % so center #1
      /                                         % and print /
   \fi}
\newcommand{\dslash}{\slashchar{\partial}}
\newcommand{\Dslash}{\slashchar{D}}

\newcommand{\eg}{\textsl{e.g.}\;}
\newcommand{\ie}{\textsl{i.e.}\;}
\newcommand{\etal}{\textsl{et al}\;}
%\DeclareMathOperator{\tr}{Tr}

% maximal number of floating environments on each page 
\setlength{\floatsep}{0pt}
\setcounter{topnumber}{1}
\setcounter{bottomnumber}{1}
\setcounter{totalnumber}{1}
\renewcommand{\topfraction}{1.0}
\renewcommand{\bottomfraction}{1.0}
\renewcommand{\textfraction}{0.0}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\newcommand{\rig}{\rightarrow}
\newcommand{\lrig}{\longrightarrow}
\renewcommand{\d}{{\text{d}}}
\newcommand{\gl}[1]{(\ref{#1})}
\newcommand{\ta}[2]{ \frac{ {\text{d}} #1 } {{\text{d}} #2}}
\newcommand{\ep}{\varepsilon}
\newcommand{\eps}{\epsilon}
%\renewcommand{\vec}{\bf}
\newcommand{\emt}{$\times 10^{-3}$}
\newcommand{\emfo}{$\times 10^{-4}$}
\newcommand{\emfi}{$\times 10^{-5}$}

\newcommand{\revision}[1]{{\bf{}#1}}

\newcommand{\hzero}{\ensuremath{h^0}}
\newcommand{\Hzero}{\ensuremath{H^0}}
\newcommand{\Azero}{\ensuremath{A^0}}
\newcommand{\PHiggs}{\ensuremath{H}}
\newcommand{\PW}{\ensuremath{W}}
\newcommand{\PZ}{\ensuremath{Z}}

\newcommand{\sw}{\ensuremath{s_w}}
\newcommand{\cw}{\ensuremath{c_w}}
\newcommand{\swd}{\ensuremath{s^2_w}}
\newcommand{\cwd}{\ensuremath{c^2_w}}

%% 2HDM Higgs masses
\newcommand{\mhhd}{\ensuremath{m^2_{\Hzero}}}
\newcommand{\mhh}{\ensuremath{m_{\Hzero}}}
\newcommand{\mlhd}{\ensuremath{m^2_{\hzero}}}
\newcommand{\Mlh}{\ensuremath{m_{\hzero}}}
\newcommand{\mad}{\ensuremath{m^2_{\Azero}}}
% \newcommand{\ma}{\ensuremath{m_{\Azero}}}
\newcommand{\mhpd}{\ensuremath{m^2_{\PHiggs^{\pm}}}}
\newcommand{\mhp}{\ensuremath{m_{\PHiggs^{\pm}}}}

\newcommand{\sa}{\ensuremath{\sin\alpha}}
\newcommand{\ca}{\ensuremath{\cos\alpha}}
\newcommand{\cad}{\ensuremath{\cos^2\alpha}}
\newcommand{\sad}{\ensuremath{\sin^2\alpha}}
\newcommand{\sbd}{\ensuremath{\sin^2\beta}}
\newcommand{\cbd}{\ensuremath{\cos^2\beta}}
\newcommand{\cb}{\ensuremath{\cos\beta}}
\renewcommand{\sb}{\ensuremath{\sin\beta}}
\newcommand{\tanbd}{\ensuremath{\tan^2\beta}}
\newcommand{\cotbd}{\ensuremath{\cot^2\beta}}
\newcommand{\tanb}{\ensuremath{\tan\beta}}
\newcommand{\tb}{\ensuremath{\tan\beta}}
\newcommand{\cotb}{\ensuremath{\cot\beta}}

\newcommand{\Sherpa}{S\protect\scalebox{0.8}{HERPA}\xspace}

\newcommand{\brinv}{\ensuremath{BR_{\text{inv}}}\xspace}
\newcommand{\vegas}{\texttt{Vegas}\xspace}
\newcommand{\madgraph}{\texttt{MG5aMCNLO}\xspace}
\newcommand{\pythia}{\texttt{Pythia}\xspace}
\newcommand{\fastjet}{\texttt{FastJet}\xspace}
\newcommand{\delphes}{\texttt{Delphes}\xspace}
\newcommand{\sherpa}{\texttt{Sherpa}\xspace}
\newcommand{\sklearn}{\texttt{scikit-learn}\xspace}
\newcommand{\keras}{\texttt{Keras}\xspace}
\newcommand{\theano}{\texttt{Theano}\xspace}
\newcommand{\adam}{\texttt{Adam}\xspace}
\newcommand{\etmiss}{\ensuremath{E_T^{\text{miss}}}\xspace}
\newcommand{\lumi}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\sqrts}{\ensuremath{\sqrt{s}}\xspace}


